MultiTASC++: A Continuously Adaptive Scheduler for Edge-Based Multi-Device Cascade Inference

Cascade systems, consisting of a lightweight model processing all samples and a heavier, high-accuracy model refining challenging samples, have become a widely-adopted distributed inference approach to achieving high accuracy and maintaining a low computational burden for mobile and IoT devices. As intelligent indoor environments, like smart homes, continue to expand, a new scenario emerges, the multi-device cascade. In this setting, multiple diverse devices simultaneously utilize a shared heavy model hosted on a server, often situated within or close to the consumer environment. This work introduces MultiTASC++, a continuously adaptive multi-tenancy-aware scheduler that dynamically controls the forwarding decision functions of devices to optimize system throughput while maintaining high accuracy and low latency. Through extensive experimentation in diverse device environments and with varying server-side models, we demonstrate the scheduler's efficacy in consistently maintaining a targeted satisfaction rate while providing the highest available accuracy across different device tiers and workloads of up to 100 devices. This demonstrates its scalability and efficiency in addressing the unique challenges of collaborative DNN inference in dynamic and diverse IoT environments.

==> sections/6_conclusion.tex <==
In this paper, we presented \tool, a dynamic scheduler designed to address the challenges of congestion in collaborative DNN inference involving a multitude of IoT devices in indoor intelligent spaces. By introducing the concept of the multi-tenant cascade, we have achieved continuous dynamic adaptation of threshold values, optimizing the trade-off between accuracy and service-level objectives during runtime.
\ITUpar
Our experimental evaluation, spanning diverse device environments and server-side models, has demonstrated the efficacy of our dynamic scheduler. Moreover, these experiments comparing \tool to our old implementation, led us to the conclusion that the SLO satisfaction rate updates are critical for precisely adhering to the targets set by each device. Equally essential is the adoption of continuous threshold values, paired with a method designed to counteract slow updates, for the scheduler to achieve its full potential. The harmonic cooperation between all \changed{of} these components led to a scheduler characterized by its consistent ability to maintain the satisfaction rate that is targeted, as well as allowing for system throughput to scale, while simultaneously enhancing performance across various device tiers and workloads, surpassing the abilities of its predecessor, MultiTASC.
\ITUpar
Moreover, the implementation of model switching has proven effective, allowing for the scheduler to adapt to scenarios where a different server-hosted model leads to greater efficiency.
\ITUpar
Lastly, by emulating a realistic deployment scenario with intermittent partial participation of devices, we demonstrated our dynamic scheduler's versatility, which can adapt to dynamic device availability and tune the execution configuration in a timely manner. This adaptability is vital for optimizing system performance and ensuring that the service-level objectives are met.
\ITUpar
\changed{While image classification is a well-explored and commonplace task, it would be of interest for future research to shift attention towards other significant tasks, such as speech recognition. Furthermore, the proposed system could be extended by investigating the new challenges of generative inference tasks, such as image and text generation, and designing novel methods in order to enable their deployment in multi-device cascade setups.}


